Understanding the AI-powered Binary Code Similarity Detection

AI-powered binary code similarity detection (BinSD), which transforms intricate binary code comparison to the distance measure of code embedding through neural networks, has been widely applied to program analysis. However, due to the diversity of the adopted embedding strategies, evaluation methodologies, running environments, and/or benchmarks, it is difficult to quantitatively understand to what extent the BinSD problem has been solved, especially in realworld applications. Moreover, the lack of an in-depth investigation of the increasingly complex embedding neural networks and various evaluation methodologies has become the key factor hindering the development of AI-powered BinSD. To fill these research gaps, in this paper, we present a systematic evaluation of state-of-the-art AI-powered BinSD approaches by conducting a comprehensive comparison of BinSD systems on similar function detection and two downstream applications, namely vulnerability search and license violation detection. Building upon this evaluation, we perform the first investigation of embedding neural networks and evaluation methodologies. The experimental results yield several findings, which provide valuable insights in the BinSD domain, including (1) despite the GNN-based BinSD systems currently achieving the best performance in similar function detection, there still exists considerable space for improvements;(2) the capability of AI-powered BinSD approaches exhibits significant variation when applied to different downstream applications;(3) existing evaluation methodologies still need substantial adjustments. For instance, the evaluation metrics (such as the widely adopted ROC and AUC) usually fall short of accurately representing the model performance of the practical use in realworld scenarios. Based on the extensive experiments and analysis, we further provide several promising future research directions.

==> framework.tex <==
% \section{Design of \sys}
\section{Evaluation Framework}
\label{s:design}
 To bridge the gap of the lack of comprehensive binary similarity detection benchmarks, we have created a set of representative datasets for both the basic block level and function level binary similarity detection tasks with different graph sizes and binary complexity to evaluate effectiveness and robustness of the state-of-the-art {\BCSDtool}s. %Furthermore, to facilitate the  delineates the workflow of \sys.

\subsection{Binary Code Similarity Detectors}
\label{sub:usable-BCSD}

In this paper, we focus on the AI-powered \BCSD approaches, which take the advantages of machine learning to boost the development of binary similarity analysis. Depending on the specific downstream applications, the \BCSD granularities can be various, including binary basic block comparison (used to solve code containment problem), binary function comparison (used to detect vulnerable functions), and the whole binary comparison (used to perform malware analysis). We mainly evaluate existing \BCSD approaches at the function level: providing a pair of binary function, considering whether they are equivalent. Namely, despite the significant binary change brought by the compiled architectures, optimization levels, and toolchains,  these \BCSD approaches determine whether the compared two binary functions are compiled from the same source code. We focus on these \BCSD approaches that compare binary functions because most \BCSD researches target the function level comparison.

Moreover, machine learning has boosted the applications of many AI-powered \BCSD approaches. It is impractical  and unnecessary to perform comprehensive evaluation for all of them since many \BCSD approaches base on the similar techniques with limited variations. To avoid redundant comparison and reduce reviewer's effort for problem understanding, the \BCSD approaches evaluated in this paper represent the latest binary function embedding skills including various binary feature extraction methods, code representation manners, and embedding neural network types.
%
Finally, as shown in~\autoref{tab:BCSD-comparision},  to date we evaluate 20 \BCSD tools including 17 academic approaches in our study. 
%and 3 commody tools including Darungrim~\cite{Darungrim}, Diaphora~\cite{Diaphora}, and Bindiff~\cite{Bindiff} 

\KL{A brief overview of the following tools.} 

\textbf{Asm2Vec}. We evaluate Asm2Vec~\cite{ding2019asm2vec}, the only approach in the investigated systems that proposes to represent the control flow graph as multiple linearly laid-out assembly sequences, which models the potential execution traces of a binary function by a random walk. After randomized ordering, these sequences are input into a representation learning model to learn the semantics of assembly code by maximizing the pre-defined log probability across a function repository (a classic document representation generation approach in NLP). However, we observe that such code representation 

\textbf{Asteria}. 
We perform an in-depth analysis of Asteria~\cite{yang2021asteria}. When selecting the structural representations of binary code, Asteria demonstrates that the binary abstract syntax tree (AST) extracted by disassembly tools such as IDA-Pro shows better stability across different architectures. Thus, the ASTs of different binaries that are compiled from the same source code tend to be the same, which is beneficial for binary code similarity detection. Then, through a Tree-LSTM~\cite{tai2015improved}, which preserves the advantages of LSTM gating mechanisms while can process the tree-structured objects, Asteria converts an AST to a representative function embedding. Unfortunately, though the ASTs of binaries compiled from the same source code trend to be the same, the ASTs of binaries compiled from difference sources may also happen to be identical.

\textbf{BinaryAI}. 
%We find that in the binary feature selection phase, similar to \textit{Focus}, BinaryAI also adopt the semantics-contained instruction embedding . 
We also benchmark BinaryAI~\cite{yu2020order}. Different from other representation learning models, BinaryAI adopts the embedding concatenation skill~\cite{mello2021use} to capture as much useful program information as possible. Namely, MPNN~\cite{gilmer2017neural} is used to generate the binary graph semantic embedding, while CNN~\cite{albawi2017understanding} is adopted to extract the graph order embedding. Finally, a function embedding is represented by concatenating them with an MLP~\cite{taud2018multilayer} layer. However, such embedding concatenation raises the weight of CFG structural information, which may make the neural network overly focuses on the node ordering of binary CFG while ignoring the graph semantics. Thus,  we perform an in-depth evaluation on BinaryAI to understand how the order of the CFG’s nodes affects a binary embedding neural network in ~\autoref{}.

\textbf{Gemini}. We benchmark Gemini~\cite{xu2017neural}, a well-known binary code similarity detector that is used as the baseline in most academic research. Gemini performs manual features extraction (MFE) according to expert knowledge and aims to select binary attributes that remain the same cross-architecture, cross-optimization, and cross-compiler settings. However, our study reveals that it lacks fool-proof support for feature selection, i.e. the manually selected features do not always remain the same for binaries compiled from different ISAs, optimization levels, and compilers. For instance, .  
     
In the embedding generation process, Gemini uses parameterized Structure2vec~\cite{dai2016discriminative}, a graphical model inference algorithm that aggregates node features to represent the whole graph embedding since each vertex, as the component, represents the graph characteristics. However, the experimental findings in ~\autoref{} show that such aggregation may cause the problem of collision, which will be further discussed in. 

%\textbf{MGMN}.

\textbf{Focus}. We also study a recently-released binary code similarity detector \textit{Focus}~\cite{fu2021focus}. Different from Gemini, in the feature engineering process, instead of extracting binary attributes according to the expert-defined pattern, \textit{Focus} directly extracts the semantics of assembly instructions by mimicking NLP tasks~\cite{Mikolov2013Distributed}. Besides, when performing binary embedding, \textit{Focus} applies the multi-head attention mechanism~\cite{velivckovic2017graph} on the graph neural network~\cite{dai2016discriminative} to construct a  semantic-aware GTN, which can selectively capture the critical features of a binary code snippet to help generate more representative binary embeddings. 

%\textbf{FuncSim}. We also evaluate %FuncSim\footnote{https://github.com/googleprojectzero/functionsimsearch/}, a C++ toolkit with python bindings, which provides a hash function (based on SimHashing~\cite{SimHash}) to  calculate a 128-bit hash  for the disassembled binary functions to ensure a good fuzzy matching performance.  The binary features selected by FuncSim are subgraphs of CFG and n-grams of mnemonics of disassembled instructions. FuncSim adopts L-BFGS~\cite{LBFGS}, a popular algorithm for parameter estimation in machine learning to investigate the weights of good program features that will be preserved across compiler changes.

% \textbf{BinDiff}. Except for academic \BCSD approaches, we also evaluate a representative binary diffing tool BinDiff which is the de facto standard approach used in industry/academy as a plugin in IDA disassembler or the baseline in many researches~\cite{duan2020deepbindiff,bourquin2013binslayer,xu2017spain,liu2018alphadiff,shirani2018binarm,chandramohan2016bingo}. BinDiff adopts graph isomorphism theory to perform binary CFG  diffing across architectures, which has been widely adopted in malware analysis system, vulnerability detection, and patch identification on both Windows and Linux.

We indeed spend considerable manual effort to investigate the remaining \BCSD tools described in~\autoref{tab:BCSD-comparision}. Considering that (1) for part of \BCSD systems, the feature selection method and the design of embedding network actually do not change much; For instance, the overall design of UFI is similar to \textit{Focus}. And (2) the great manual effort spent in the analysis of \BCSD approaches when applied to downstream applications. We choose to perform comprehensive and in-depth analysi for the above 7 representative binary similarity detectors, which include all the embedding networks described in~\autoref{s:preliminaries}.    
 
%  we further explore cross-architecture, cross-optimization, and cross-compiler settings, 
 
\subsection{Evaluation Datasets}
\label{sub:eval-dataset}
%\BCSD 
To achieve the goal of comprehensively comparing \BCSD approaches on both general binary diffing and two representative downstream applications (vulnerability search and license violation detection), we carefully prepare two representative datasets, which are\KL{will be?} publicly available.
\KL{it is important to explain how you prepare these datasets and why these two datasets are great }

\textbf{Dataset-1}\KL{better give it a name}: Dataset-1 is the benchmark binary programs used to train the evaluated AI-powered \BCSD systems and perform general binary diffing, i.e., function search utilities. On this dataset, similar to prior researches, we evaluate the AUC and ACC values of the training neural networks and calculate multiple function searching rank metrics such as MAP, MRR, NDCG, and so on.
%
Indeed, many prior researchers have proposed their own benchmark dataset. However, most datasets used in prior works are not open-sourced. Moreover, existing datasets are either too small, which only contain several binaries compiled under limited architectures or optimization levels, or too large, which includes many reduplicate binaries that do not actually benefit the model training process but make the overall evaluation time to be long and unacceptable.
%
According to our investigation of existing \BCSD researches, we observe that the complexity (defined in this paper including assembly size, the number of basic blocks, and the number of the contained callee functions), architecture, and optimization level of binary can greatly influence the overall performance of a \BCSD system. Thus, as a suitable and representative benchmark, we expect dataset-1 to contain suitable numbers of binaries that presents various complexity, function utilities, architectures, and optimization levels. 
%and contains binaries of various complexity (here we define complexity to be the length of assembly instructions, the number of vetex and edges of the CFG, and number of callee functions within this function.)  

Based on the binaries released by \textsc{BinKit}~\footnote{https://github.com/SoftSec-KAIST/BinKit}, we duplicate binaries that show the same complexity and add extra binaries present new program complexity or function utilities. Specifically, as shown in~\autoref{fig:subfig1},~\autoref{fig:subfig2}, and~\autoref{fig:subfig3}, the distribution of basic blocks, callees, and number of assembly are similar for the four presented binaries. Thus, we only keep one of them in dataset-1. As for architectures, it is unnecessary and infeasible to include all the architectures. The root reason is that as shown in~\autoref{tab:BCSD-comparision},  the architectures that existing \BCSD approaches support various a lot. It is impractical to reimplement all the existing \BCSD approaches to support all the architectures. Thus, considering the architectures that existing \BCSD approaches support and the difficulty of \BCSD cross-architectures, we evaluate binaries compiled under three architecture, x86, x64, and arm. The reason is that as show in~\autoref{fig:comparision-across-different-architectures}, the binary diffing between x86 and x64 is the easiest one while the binary comparison between x86 and arm is the most difficult one. As for optimization levels,  we include 4 popular optimization levels (-O0-O3).
%
Finally, as shown in~\autoref{tab:software},  we carefully select 27 open-source programs, which contain XX distinct executable, and XX functions. The distribution of assembly size, the number of basic blocks, and the number of the contained callee functions are shown in XX. 
%Each binary file is compiled under three architecture, x86, x64, and arm and 4 optimization levels (-O0-O3). These three architectures are carefully select according to (1) the architectures that existing \BCSD approaches support and (2) the binary diffing between x86 and x64 is the easiest one while the binary comparison between x86 and arm is the most difficult one. 
Particularly, dataset-1 is divided into two group to evaluate embedding neural networks on both seen and unseen binaries (the binary with * in~\autoref{tab:software}).

\textbf{Dataset-2}:  Dataset-2 is used to validate the effectiveness of existing \BCSD approaches on downstream real-world applications.
%vulnerability search and license violation detection. 
Similar to prior researches, we also perform this evaluation on the most common scenarios: vulnerability search in IoT firmware. Considering the difficulty of vulnerability search varies for different types of vulnerabilities, we collect XX vulnerable functions in widely spread third-party libraries such as openssl, busybox, and gzip. These XX vulnerabilities consist of missing security check, missing variable initialization, double free.  Intuitively, missing security check usually alter the CFG of binaries, which is more easier to be identified than other two types of vulnerabilities. As for the IoT firmware that need to be checked,  we randomly choose 20 representative IoT firmware from four leading IoT vendors (DLink, TPLink, Tuya, and trendnet) of various utilities including switch, router, IP-camera and access point. In this evaluation, we do not plan to perform a large-scale bug detection to investigate the security state of a large amount of IoT firmware. By contrast, we aim to validate the true of capabilities of  AI-powered \BCSD approaches. Thus, 20 IoT firmware that include XX binaries and XX functions is suitable for this evaluation within acceptable time.
%
. As for license violation detection, we check whether the select 20 IoT firmware use the open-source third libraries such as openssl and busybox.
% To bridge the gap of the lack of standard evaluation datasets, we gather three representative datasets for binary similarity detection, including 
% The complexity of graph (the number of the instructions, basic blocks, called functions within a function, and density). 
\subsection{Evaluation Metrics}
\label{sub:eval-metric}
Inadequate evaluation metrics may lead to an understanding trap. Thus, it is important to shed light on the pros and cons of the machine learning metrics, which help to fairly measure state-of-the-art \BCSD approaches. In this section, we first introduce existing evaluation metrics that have ever been used in the investigated \BCSD approaches. Furthermore, we perform a comprehensive analysis and comparison of the described machine learning metrics, which help us to determine the suitable and sufficient metrics for \BCSD.
% based on our heuristic analysis on the problem of binary similarity detection, we also summarize and propose several evaluation metrics, which serve as a complementary of existing evaluation metrics. In the following, we present concrete metrics.

\begin{figure*}[htbp]
    \begin{minipage}[t]{0.32\linewidth}
        \centering
            \subfloat[coreutils-nproc]{
                \label{fig1a} 
                \includegraphics[width=0.49\linewidth]{fig/binary_selection/coreutils_coreutils-8.29_gcc-6.4.0_x86_64_O1_nproc.elf_bbs_edge.pdf}}
            \subfloat[findutils-frcode]{
                \label{fig1b} 
                \includegraphics[width=0.49\linewidth]{fig/binary_selection/findutils_findutils-4.6.0_gcc-6.4.0_x86_64_O1_frcode.elf_bbs_edge.pdf}}
            \vfill
            \subfloat[inetutils-dns*]{
                \label{fig1c} 
                \includegraphics[width=0.49\linewidth]{fig/binary_selection/inetutils_inetutils-1.9.4_gcc-6.4.0_x86_64_O1_dnsdomainname.elf_bbs_edge.pdf}}
            \subfloat[inetutils-rexec]{
                \label{fig1d} 
                \includegraphics[width=0.49\linewidth]{fig/binary_selection/inetutils_inetutils-1.9.4_gcc-6.4.0_x86_64_O1_rexecd.elf_bbs_edge.pdf}}
            \caption{The distribution of basic blocks and edges}
            \label{fig:subfig1}
    \end{minipage}
\hfill
    \begin{minipage}[t]{0.32\linewidth}
        \centering
            \subfloat[coreutils-nproc]{
                \label{fig2a} 
                \includegraphics[width=0.49\linewidth]{fig/binary_selection/coreutils_coreutils-8.29_gcc-6.4.0_x86_64_O1_nproc.elf_funcCalls.pdf}}
            \subfloat[findutils-frcode]{
                \label{fig2b} 
                \includegraphics[width=0.49\linewidth]{fig/binary_selection/findutils_findutils-4.6.0_gcc-6.4.0_x86_64_O1_frcode.elf_funcCalls.pdf}}
            \vfill
            \subfloat[inetutils-dns*]{
                \label{fig2c} 
                \includegraphics[width=0.49\linewidth]{fig/binary_selection/inetutils_inetutils-1.9.4_gcc-6.4.0_x86_64_O1_dnsdomainname.elf_funcCalls.pdf}}
            \subfloat[inetutils-rexec]{
                \label{fig2d} 
                \includegraphics[width=0.49\linewidth]{fig/binary_selection/coreutils_coreutils-8.29_gcc-6.4.0_x86_64_O1_nproc.elf_funcCalls.pdf}}
            \caption{The distribution of FuncCalls}
            \label{fig:subfig2}
    \end{minipage}
\hfill
    \begin{minipage}[t]{0.32\linewidth}
        \centering
            \subfloat[coreutils-nproc]{
                \label{fig3a} 
                \includegraphics[width=0.49\linewidth]{fig/binary_selection/coreutils_coreutils-8.29_gcc-6.4.0_x86_64_O1_nproc.elf_inst_size.pdf}}
            \subfloat[findutils-frcode]{
                \label{fig3b} 
                \includegraphics[width=0.49\linewidth]{fig/binary_selection/findutils_findutils-4.6.0_gcc-6.4.0_x86_64_O1_frcode.elf_inst_size.pdf}}
            \vfill
            \subfloat[inetutils-dns*]{
                \label{fig3c} 
                \includegraphics[width=0.49\linewidth]{fig/binary_selection/inetutils_inetutils-1.9.4_gcc-6.4.0_x86_64_O1_dnsdomainname.elf_inst_size.pdf}}
            \subfloat[inetutils-rexec]{
                \label{fig3d} 
                \includegraphics[width=0.49\linewidth]{fig/binary_selection/inetutils_inetutils-1.9.4_gcc-6.4.0_x86_64_O1_rexec.elf_inst_size.pdf}}
            \caption{The distribution of FuncSize}
            \label{fig:subfig3}
    \end{minipage}
\end{figure*}




% \subsubsection{Existing Evaluation Metrics}
% \label{subsub:existing-eval-metric}
%\begin{itemize}
% \PP{ROC curve}  Receiver operating characteristics (ROC) curve is one of the most important metrics for a binary classification model, which is also the most prevalent adopted metric in binary similarity detectors. ROC curve is a probability curve where the x-axis and the y-axis represent the false positive rate (FPR) and true positive rate (TPR) at different threshold settings, respectively.  The FPR and TPR are defined as below:

% \begin{equation}\label{algrithm-fpr}
% 	FPR = \frac{FP}{FP + TN}
% \end{equation}

% \begin{equation}\label{algrithm-tpr}
% 	TPR = \frac{TP}{ TP + FN }
% \end{equation}

% \PP{AUC} AUC is the area under the ROC curve. % which can directly be used to compare the performance of classifiers.  Specifically 
% The higher the AUC value, the better the model is at distinguishing binary code from different source code.

% \PP{F1 score} F1 score represents the weighted average of Precision and Recall, which considers both false positives and false negatives. Thus, F1 score is suitable to evaluate the models that have uneven class distribution.
% \begin{equation}\label{algrithm-presicion}
% Precision = \frac{TP}{ TP + FP }
% \end{equation}

% \begin{equation}\label{algrithm-recall}
% Recall = \frac{TP }{ TP + FN }
% \end{equation}

% \begin{equation}\label{algrithm-f1-score}
% F1\_score = \frac{ 2*(Precision * Recall  )}{ Precision + Recall }
% \end{equation}


% \PP{Precision@K} Precision@K represents the fraction of relevant searching results  (the repository function are compiled from the same source code as query function) in the top K ranking list. asm2vec evaluates the performance of the proposed model by using Precision@1.

% \PP{MRR} Similar to recommendation systems, given a query function, binary similarity detection approaches eventually output a ranking list of repository functions. Thus, we need a metric to evaluate the ranking quality. Mean reciprocal rank (MRR) can provide a general measurement of the quality of the searching results, which is appropriate to judge the performance of a model when we only care about the highest-ranked searching results. MRR can be calculated according to equation~\ref{algrithm-mrr} where Q is the number of the queries and relevance score is either 0 or 1 (0 means the query function and the corresponding repository function are not compiled from the same source code. By contrast, if the query function and  the repository function are compiled from the same source code, the relevance score is 1.) $rank_i$ refers to the rank position of the first relevant function for the i-th query
% \begin{equation}\label{algrithm-mrr}
% 	MRR = \frac{1}{|Q|} \sum_{i = 1}^{|Q|}\frac{relevance_i}{rank_i}
% \end{equation}

% %\item{\bf Recall@K:} Recall@K represents the fraction of relevant searching result   
% \PP{NDCG} NDCG  refers to normalized discounted cumulative gain, in which gain is similar to the relevance score in MRR. I(Q) is  the ideal discounted cumulative gain.
% \begin{equation}\label{algrithm-dcg}
% 	DCG(Q) =   \sum_{i = 1}^{Q}\frac{relevance_i}{log_2(i+1)}
% \end{equation}

% \begin{equation}\label{algrithm-idcg}
% 	IDCG(Q) =  \sum_{i = 1}^{|I(Q)| }\frac{relevance_i}{log_2(i+1)}
% \end{equation}

% \begin{equation}\label{algrithm-ndcg}
% 	NDCG(Q) =  \frac{DCG(Q)}{IDCG(Q)}
% \end{equation}

% \PP{Recall@K} Recall@K represents the fraction of relevant searching result in all the relevant repository functions.

% \PP{Rank1} indicates whether the top-1 searching result, i.e. the one that has the highest similarity score is compiled from the same source as the query function.


% \begin{equation}\label{algrithm-ndcg}
% 	Rank1 =  \frac{T}{Q}
% \end{equation}
% where Q is the time of function query, T is the times that the top1 searching result is the binary compiled from the same source as the query function. 

% \PP{MAP} Mean average precision (MAP) examines a new sub-list every time we meet a new relevant similar function to calculate the precision and average the precision to obtain average precision AveP(q)

% \begin{equation}\label{algrithm-ndcg}
% 	MAP =  \frac{\sum_{q = 1}^{Q}(AveP(q))}{Q}
% \end{equation}

%\end{itemize}

AUC and ROC are discrimination index used to evaluate the performance of classifiers, which represents the likelihood that similar functions compiled from the same source code have higher similarity score than randomly generated dissimilar functions pairs. Unfortunately, good discrimination power does not mean good fitted model.

Precision@K, recall@K and F1 score@K help users select more "relevant" similar function, and avoid "irrelevant" ones, which starts to emphasize what is important for binary embedding systems. The F1 score metric is used to balance precision and recall. \textbf{However, these metrics do not care about the rank of "relevant"  searching results.} For instance, no matter the "relevant" similar function in the first one or the last one position, the Precision@K, recall@K and F1 score@K are the same.

The primary concern of a good \BCSD tool is to report the "relevant" similar functions very high up the list of searching results.
MRR, MAP, and NDCG are popular rank-aware metrics used in recommendation systems, which can be adopted in our scenario. MRR mainly focuses on the first relevant similar function in the searching list. Only when the first relevant similar function ranks highly, MRR will be high, which is not a good evaluation metric when there is a list of related functions to check. MAP heavily weights the error at the top of searching results, which shines for binary rating by presenting the complex area under the precision-recall curve. NDCG provides a logarithm reduction factor to proportionally penalize the relevant score to the position of searching functions. Moreover, NDCG normalizes this metric between 0 and 1 to avoid incomparable DCG. Compared to MAP, the logarithm reduction factor of NDCG has a good theoretical basis, which enable this metric consistently select the better system~\cite{wang2013theoretical}.
\KL{so how do you plan to actually select and integrate them? How the selection can be more systematic or
even automated?}

==> name.tex <==
AI-powered binary code similarity detection (BinSD), which transforms binary diffing to the comparison of code embedding through neural networks, has been widely applied to program analysis. However, it is still unclear whether the state-of-the-art AI-powered code embedding neural networks and evaluation methodologies are suitable for BinSD, due to the lack of in-depth understanding of the increasingly complex and various embedding neural networks, as well as the inconsistency of the adopted embedding strategies, evaluation methodologies, running environments, and benchmarks. 
It is also unknown how existing AI-powered BinSD tools compare to each other and perform in the downstream applications. 

To fill these research gaps, in this paper, we present the first systematic evaluation of state-of-the-art AI-powered BinSD approaches by performing an in-depth analysis and comprehensive BinSD system comparison on both general binary diffing and two representative downstream applications, namely vulnerability search and license violation detection. We aim for meaningful and fair  evaluation by using the same evaluation methodologies (evaluation metrics and datasets). The experimental results show that (1) The current usage of some embedding neural networks (such as graph neural networks and convolutional neural networks) does not fit well in BinSD by nature. (2) Existing evaluation methodologies still need significant adjustments. For instance, the evaluation metrics (such as ROC and AUC)  are insufficient to represent the performance of the practical usage in real-world scenarios. (3) There exists a huge space for improvement for AI-powered BinSD approaches. Moreover, the capability of existing AI-powered BinSD approaches varies when applied to different downstream applications. We provide several promising future directions based on the in-depth analysis and comprehensive experimental results. To facilitate the reproducibility of our findings, we will release all the datasets, benchmarks, and implementation as docker images. 

==> relwk.tex <==
%\section{Technical Background}
\section{ Background}
\label{s:preliminaries}


The AI-powered \BCSD approaches are often built on different techniques and complex neural networks. To better understand existing AI-powered \BCSD approaches, we summarize their mainstream workflow in~\autoref{workflow-of-BCSD}.
The workflow usually consists of three phases: preprocessing, code representation, and network embedding.  
Note that not every \BCSD approach has all these phases. 

\subsection{Phases of \BCSD}
\label{phaseofBCSD}
 \textbf{Preprocessing.} %The ultimate goal of AI-powered \BCSD approaches is to transform binaries into low-dimensional code embedding. During the transformation process, researchers expect the binary change of two binary code snippets compiled from the same source code to be as small as possible. The root reason is that small binary changes benefit the embedding networks to generate similar code embeddings. Moreover, researchers would like to extract representative binary features to differentiate unrelated binaries.  
%
Given two binary code snippets in the first phase, the AI-powered \BCSD tools usually perform binary feature extraction. Specifically, after code disassembly, most \BCSD approaches~\cite{duan2020deepbindiff, fu2021focus, massarelli2018safe, zuo2018neural} perform instruction normalization to avoid the out-of-vocabulary (OOV) problem~\cite{bazzi2002modelling} (a common issue in NLP). Besides, some \BCSD tools~\cite{chandramohan2016bingo, ding2019asm2vec} perform selective callee inline to decrease the CFG change brought by function inlining.
Several other \BCSD tools~\cite{xu2017neural, gao2018vulseeker} perform manual feature extraction or instruction embedding~\cite{massarelli2018safe, fu2021focus, yu2020order} to obtain binary features as the unique label of binaries. %input of embedding networks.

\textbf{Code representation.} After pre-processing, intuitively, one needs to consider the specific binary code representation
as the input of embedding neural networks. According to our empirical analysis, the AI-powered BinSD tools usually represent a binary code snippet as a basic block adjacent matrix, sequential instruction sequences, abstract syntax tree (AST), control flow graph (CFG), data flow graph (DFG), or the combinations of them.
 

\textbf{Network embedding.}  Finally, based on the widely used neural networks such as CNN and GNN, existing AI-powered \BCSD approaches convert specific code representation % together with the binary features 
to low-dimensional vector---code embedding, which will be further compared to determine the similarity score of the input binary code pairs. It is worth noting that the technique difference of some existing AI-powered \BCSD approaches in the three phases is minor. For instance, compared to Gemini~\cite{xu2017neural}, except for CFG, VulSeeker~\cite{gao2018vulseeker} also extracts DFG when performing code representation.
%
Next, we briefly introduce the mainstream embedding neural networks used in the state-of-the-art \BCSD approaches.
%\begin{itemize}
%
%\item
% \subsection{Mainstream Embedding Neural Networks}

% {\bf NLP-based models.} 
% After binary code disassembling, a binary code snippet can be represented using an assembly language, which to some extent shares many analogical topics with a natural language---both of them are organized by specific grammatical structures and can express certain semantics. Therefore, when embedding the obtained instruction sequences, many studies propose to treat instructions as words, functions as sentences, and the whole binaries as paragraphs in natural language. Then, researchers turn to converting the assembly language into low-dimensional vectors in the same way as NLP tasks. For instance, Asm2Vec~\cite{ding2019asm2vec} uses an improved PV-DM model~\cite{le2014distributed}, an unsupervised NLP learning approach, to generate code embedding for binary functions. 

% %\item
% {\bf RNN/LSTM-based models.} 
% Recursive Neural Networks (RNN) and LSTM (a special RNN with gate mechanisms)~\cite{Greff2017LSTM} have been proven to be effective in sentiment analysis, language translation, and question answering. Thus, many studies turn to applying RNN/LSTM models to extract the semantics of binary code. For instance, \textsc{InnerEye}~\cite{zuo2019neural} proposes to use neural machine translation (NMT), a kind of LSTM model, to detect basic block similarity. Asteria~\cite{yang2021asteria} and SAFE~\cite{massarelli2018safe} use LSTM/RNN  to learn the semantic representation of a binary function. 

% %\item
% {\bf CNN-based models.} 
% CNN~\cite{albawi2017understanding} has been widely applied to image and video recognition, classification, and processing, which is good at grasping node connectivity patterns in matrix data through kernels. Considering (1) the raw bytes contain all the semantics of binary code, and (2) the node order of the CFGs of binaries (adjacent matrices) compiled from the same source code is highly likely to remain the same, researchers proposed to learn the raw bytes pattern or the \textit{node order information} of CFGs by CNN, which can be used as an important program feature in binary code similarity detection. For example, BinaryAI~\cite{yu2020order} uses a 3-layer CNN to construct an order-aware model to learn function embedding. $\alpha$Diff~\cite{liu2018alphadiff} represents the raw bytes of binary code as a matrix and then uses a CNN to generate function embeddings. 
 
% %\item
% {\bf GNN-based models.} 
% %Recently, there has been a surge of interest in neural graph networks (GNN), a powerful class of deep learning models that yield effective representation for structured objects. Various of GNNs have been proposed for learning effective graph embedding vectors. 
% Using disassembling tools such as IDA~\cite{ida-pro-7-0} and Radare2~\cite{radare2}, one can obtain the graph representation (CFG or DFG) of a binary code snippet. Thus, many \BCSD approaches~\cite{xu2017neural,gao2018vulseeker,Baldoni2018Unsupervised} consider using various kinds of GNNs (a powerful class of deep learning models that yield effective representation for structured objects), including Structure2Vec~\cite{dai2016discriminative}, graph attention networks~\cite{velivckovic2017graph} and graph convolution networks (GCN)~\cite{kipf2016semi, kim2022improving,luovulhawk} to learn the vector representation of binary code. For instance, Gemini~\cite{xu2017neural} improves Genius~\cite{feng2016scalable} by using Structure2Vec~\cite{dai2016discriminative} to transform binary functions into embeddings according to the corresponding CFG and manually extracted features. 
% %By leveraging both the CFG and DFG, Vulseeker~\cite{gao2018vulseeker} and Vulseeker-pro develops a deep neural network (DNN) model to extract the graph embedding vector, which can be used to represent the entire binary function semantics. 

% %\item
% {\bf Other models.} 
% Except for the above mainstream neural networks, other neural networks such as message-passing neural networks (MPNN)~\cite{gilmer2017neural} and proc2vec~\cite{shalev2018binary} are also applied to the existing AI-power \BCSD tools. For instance, BinaryAI~\cite{yu2020order} also adopts MPNN, which extracts the structural information of a binary CFG to learn the representation of binary code. In this paper, we aim to comprehensively evaluate the widely used embedding neural networks, including the NLP-based, RNN/LSTM-based,  CNN-based, and GNN-based models.
%which may be potentially more influential in the problem scope.

%\end{itemize}

\subsection{Scope}
\BCSD approaches are supposed to be used in large-scale downstream applications. In this situation, many researchers consider static analysis to ensure efficiency and avoid the problem of code coverage in dynamic analysis. Consequently, this paper aims to evaluate static \BCSD approaches. Moreover,
depending on the specific downstream applications, the \BCSD granularities vary, including binary basic block comparison (solving code containment problems), binary function comparison 
(detecting vulnerable functions), 
and the whole binary comparison (performing malware analysis). 
We mainly evaluate existing \BCSD approaches at the function level---providing a pair of binary functions, we examine whether they are similar (compiled from the same source code) because most \BCSD approaches are based on function level comparison. Finally, the analysis of the obfuscated binaries is out of our scope since most \BCSD approaches do not support obfuscated binary embedding.
